The Face of Persuasion: Analyzing Bias and Generating Culture-Aware Ads

Text-to-image models are appealing for customizing visual advertisements and targeting specific populations. We investigate this potential by examining the demographic bias within ads for different ad topics, and the disparate level of persuasiveness (judged by models) of ads that are identical except for gender/race of the people portrayed. We also experiment with a technique to target ads for specific countries. The code is available at https://github.com/aysanaghazadeh/FaceOfPersuasion

==> sections/_dump.tex <==
% With recent advancements in generative AI, a wide range of new applications have emerged. One important area is media creation, where AI models are now being used to generate content such as images, text, and videos. A growing use case within this space is advertisement generation.

% Generative models like large language models (LLMs) and Text-to-Image (T2I) models can now create advertisement content quickly and at scale. These systems can write persuasive advertisement description, generate product descriptions, or even produce advertisement scenarios based on abstract message prompts like \textit{`I should drink this beer because it is as light as feather'}. While this opens up great possibilities for faster and more personalized marketing, it also raises concerns around fairness and bias especially when targeting specific audience. 

% Advertisements, whether real or AI-generated, can contain or reinforce stereotypes related to gender, race, age, or other social categories. In some cases, biased content may even appear more persuasive because it plays into familiar social patterns or expectations. This brings up an important question: is there a correlation between how bias and persuasion?

% In this work, we explore that question by studying three types of ads: real advertisements, ads generated directly by text-to-image models, and ads created using descriptions written by LLMs. To evaluate We use both LLMs and multimodal models (MLLMs) to score each image persuasion and further extract stereotypes related to gender and race. By comparing these scores, we aim to better understand how AI-generated content reflects bias, and whether bias is linked to how persuasive an ad is perceived to be.

% One important factor in persuasion is the target audience, while an advertisement can be persuasive in one culture it might be totally neutral or even negative in another cultural. 

%two types of prompts: one based on the action-reason statements from the dataset, denoted as $I_{AR}$, and another based on textual descriptions generated by a large language model (LLM), denoted as $I_{LLM}$. We evaluate demographic bias in various text-to-image (T2I) models by generating $I_{AR}$ with each model and analyzing the demographic composition of the resulting images. In parallel, we assess bias in different LLMs by generating $I_{LLM}$ from each model’s descriptions. 

% \subsection{Bias Analysis}
% \textbf{Demographic Diversity in PittAd} PittAd dataset \cite{PittAd} is a major source of data in visual persuasive contents like advertisement images and advertisement videos. In this work we begin by evaluating the distribution of different races 
% \subsection{Cultural Ad Dataset Annotation}
% \subsection{Cultural Aware Advertisement Generation}

% \subsection{Bias in Generative AI}
% \textbf{Bias in T2I generation models and LLMs.}
% \textbf{Bias in country aware image generation}
% \textbf{Bias in MLLMs and LLMs for persuasion}
% \subsection{Data Statistics}
% \subsection{Cultural Aware Image Generation}


==> sections/_experimental_setup.tex <==
\section{Experimental Setup}

\subsection{Datasets}

\subsection{Bias Evaluation Models}

\subsection{Baseline Models}


==> sections/old_introduction.tex <==
\section{Introduction}
% With recent advancements in generative AI, a wide range of new applications have emerged. One important area is media creation, where AI models are now being used to generate content such as images, text, and videos. A growing use case within this space is advertisement generation.

% Generative models like large language models (LLMs) and Text-to-Image (T2I) models can now create advertisement content quickly and at scale. These systems can write persuasive advertisement description, generate product descriptions, or even produce advertisement scenarios based on abstract message prompts like \textit{`I should drink this beer because it is as light as feather'}. While this opens up great possibilities for faster and more personalized marketing, it also raises concerns around fairness and bias especially when targeting specific audience. 

% Advertisements, whether real or AI-generated, can contain or reinforce stereotypes related to gender, race, age, or other social categories. In some cases, biased content may even appear more persuasive because it plays into familiar social patterns or expectations. This brings up an important question: is there a correlation between how bias and persuasion?

% In this work, we explore that question by studying three types of ads: real advertisements, ads generated directly by text-to-image models, and ads created using descriptions written by LLMs. To evaluate We use both LLMs and multimodal models (MLLMs) to score each image persuasion and further extract stereotypes related to gender and race. By comparing these scores, we aim to better understand how AI-generated content reflects bias, and whether bias is linked to how persuasive an ad is perceived to be.

% One important factor in persuasion is the target audience, while an advertisement can be persuasive in one culture it might be totally neutral or even negative in another cultural. 

Generative models have demonstrated remarkable performance, particularly through training on large-scale datasets or with human feedback \cite{LLM_African}. This progress has led to their adoption in a wide range of applications, especially content generation tasks like creative and persuasive content generation \cite{wacv, cap}. 

These models can now produce persuasive content rapidly and at scale, enabling tasks such as generating advertisements, writing product descriptions, or crafting ad scenarios from abstract prompts. However, despite advances in training methods, there remain limitations in the demographic diversity of datasets and human annotators \cite{LLM_African}. These limitations raise concerns about potential bias in both the training process and the content generated. In the context of persuasive content, such bias is becomes more challenging to address due to the importance of target audience in persuasion of the content. For instance, an advertisement aimed at a Japanese audience may benefit from featuring an Asian person, whereas the same visual cue could be neutral, or even counterproductive when targeting audiences in the United Arab Emirates. But is it always necessary to include specific demographic representations to enhance persuasiveness? And what happens when the target audience is more universal or from a more demographically diverse country like United States? 
\input{figures/intro}
In this paper, we investigate bias in generative models for persuasive content using the PittAd dataset \cite{PittAd}. The PittAd dataset contains advertisement images paired with abstract message interpretations, structured as \textit{`I should \textbf{action} because \textbf{reason}'} referred to as action-reason statements. We begin by analyzing the demographic diversity represented in the dataset. Then, following the approach of \cite{CAP}, we generate advertisement images using two types of prompts: one based on the action-reason statements from the dataset, denoted as $I_{AR}$, and another based on textual descriptions generated by a large language model (LLM), denoted as $I_{LLM}$. We evaluate demographic bias in various text-to-image (T2I) models by generating $I_{AR}$ with each model and analyzing the demographic composition of the resulting images. In parallel, we assess bias in different LLMs by generating $I_{LLM}$ from each model’s descriptions. To analyze the bias in generated images demographic features were extracted by DeepFace \cite{deepface}.
Our analysis reveals that racial and gender distributions vary across advertisement topics, and that both the dataset and the generated images exhibit racial bias. Our finding show the evidence of \textbf{stereotypical representational bias}: for example, white individuals are overrepresented in advertisements centered on topic of self-esteem, while Black individuals are more frequently depicted in charity-related contexts.

To assess how demographic of the characters in the advertisements influences persuasiveness judgments in generative models, we conducted a controlled experiment. We created sets of advertisement images that were identical except for the race of the central individual. Corresponding textual descriptions were also modified only to reflect this change. These image-description pairs were then evaluated by multimodal large language models (MLLMs) and LLMs, which were prompted to select the more persuasive option using chain-of-thought (CoT) reasoning \cite{CoT}. Our findings show that MLLMs consistently favored images featuring White individuals, often justifying their choices with subjective attributes such as perceived elegance as illustrated in Fig. \ref{fig:intro}.

Many studies have shown that the target audience plays a critical role in persuasion \cite{persuasiveness}. However, given existing biases in text-to-image (T2I) models, the ability to generate advertisements tailored to different countries remains an open question. In this work, we explore this by generating advertisement images targeting specific countries. To support this, we introduce an extension to the PittAd dataset \cite{PittAd}, which includes annotations for the target country of each image as well as its cultural components. We utilize InternVL \cite{InternVL} to extract visual cultural components in the image and predict up to three likely target countries per image.
We then conduct a human evaluation on a subset of the dataset, asking annotators from diverse countries to assess the accuracy of the model’s country predictions. The results show that our annotation model achieves a recall of 81\% and a precision@1 (P@1) of 72\%. When grouping countries by similar cultural regions, these scores improve to 94\% recall and 75\% P@1, demonstrating the effectiveness of the annotation pipeline. With country-level annotations and corresponding action-reason statements, we prompt T2I models to generate advertisements explicitly targeting each specified country. Our findings indicate that including the target country as part of the generation process increases racial bias in the resulting images. More critically, we observe that while these models can relatively easily generate ads for culturally dominant regions such as Western countries they often struggle to produce coherent or culturally appropriate content for underrepresented cultures, such as those from the Middle East.

To address the challenge of generating culturally aligned advertisements, we propose Culture-aware Generator (CulGen). In this model, we first retrieve five randomly selected images from the target country that share the most similar topic to the input action-reason statement. From these images, we extract cultural components and randomly select one image to serve as a conditioning reference.
Inspired by proposed method in \cite{Rare-to-freq}, our model progressively incorporates conditioning information during the denoising process. In the early time-steps, the model is conditioned only on the prompt. In the middle time-steps, we introduce both the prompt and the extracted cultural components. Finally, in the later time-steps, we combine the prompt, extracted cultural components, and the reference image, using them together to guide the noise prediction process. Experimental results shows that CulGen improve cultural representation across a wide range of countries, including those from both overrepresented and underrepresented cultural groups.

